Strength measurement of the $E_{\alpha}^{lab}$ = 830 keV resonance in $^{22}\rm{Ne}(\alpha,n)^{25}\rm{Mg}$ reaction using a stilbene detector

The interplay between the $^{22}$Ne$(\alpha,\gamma)^{26}$Mg and the competing $^{22}$Ne$(\alpha,n)^{25}$Mg reactions determines the efficiency of the latter as a neutron source at the temperatures of stellar helium burning. In both cases, the rates are dominated by the $\alpha$-cluster resonance at 830 keV. This resonance plays a particularly important role in determining the strength of the neutron flux for both the weak and main $s$-process as well as the $n$-process. Recent experimental studies based on transfer reactions suggest that the neutron and $\gamma$-ray strengths for this resonance are approximately equal. In this study, the $^{22}$Ne$(\alpha,n)^{25}$Mg resonance strength has been remeasured and found to be similar to the previous direct studies. This reinforces an 830 keV resonance strength that is approximately a factor of three larger for the $^{22}$Ne$(\alpha,n)^{25}$Mg reaction than for the $^{22}$Ne$(\alpha,\gamma)^{26}$Mg reaction.

==> obsolete.tex <==
 neutron energies as calibrations, three gamma rays were used as independent checks on linearity and gain. They were 137Cs(0.66 MeV) and 22Na(0.51 and 1.28 MeV). Since stilbene is an organic material with very low Z constituents (carbon and hydrogen), its response to low-energy gamma rays is entirely due to Compton scattering

